Technical Report: Toward Applying Quantum Computing to Network Verification

Network verification (NWV), broadly defined as the verification of properties of distributed protocols used in network systems, cannot be efficiently solved on classical hardware via brute force. Prior work has developed a variety of methods that scale by observing a structure in the search space and then evaluating classes within the search space instead of individual instances. However, even these classification mechanisms have their limitations. In this paper, we consider a radically different approach: applying quantum computing to more efficiently solve NWV problems. We provide an overview of how to map variants of NWV problems into unstructured search problems that can be solved via quantum computing with quadratic speedup, making the approach feasible in theory to problems that are double in size (of the input). Emerging quantum systems cannot yet tackle problems of practical interest, but rapid advances in hardware and algorithm development make now a great time to start thinking about their application. With this in mind, we explore the limits of scale of the problem for which quantum computing can solve NWV problems as unstructured search.

==> ForTR.tex <==
\begin{figure}
    \centering
    \includegraphics[height=0.4\textheight]{fig/circuit_full2.png}
    \caption{Left: Detail of Quantum Circuit to implement transfer function logic.  Middle: Oracle circuit $f$ of Grover's Algorithm.  Right: Full circuit for Quantum Search Algorithm, run for one Grover iterate.}
    \label{fig:hsa_qc}
\end{figure}


\begin{figure*}
    \centering
    \includegraphics[scale=0.3]{fig/Kylie-circ-merge.png}
    \caption{Link Outage Oracle Circuit}
    \label{fig:netdice_qc}
\end{figure*}

==> removed.tex <==
\subsection{Other points about designing $f$:}

\begin{myitemize}
   
    \item $f$ is a very non-trivial function, but there is no doubt that it can be implemented classically (e.g., in a high-level language like C or C++.  This means it can be compiled down to a circuit built out of only AND, OR and NOT gates.  Since such gates can also be implemented on a quantum computer, execution of $f$ is certainly feasible.

   %% \item The "Quantum power" comes from being able to simultaneously run all $2^n$ input instances in parallel across this circuit.  Since our initial foray does not attempt to take advantage of any structure in the underlying problem our solutions are restricted to the $O(2^{n/2})$ cost from applying unstructured search.

    \item Probabilistically, if $f$ has many violating instances of returning 1, then one can repeat and with high probability get a new instance.  If the number of instances is small, we can modify $f$ each iteration we run it to obtain another violating instance, by hard coding $f$ to reject already-seen inputs that have been confirmed to evaluate to 1.
\end{myitemize}



\section{Comparison}
\begin{myitemize}  
    \item Quantum Success where Classical 
    %Not sure if this is what was in mind for this section
    As we saw in the previous examinations involving HSA and NetDice, it becomes evident that quantum computers leveraging Grover's algorithm as a subroutine can significantly accelerate the search for network problems and enhance the scale at which one can investigate targeted properties. An additional advantage lies in Grover’s unstructured search without assuming specific states, properties, or configurations of the network, unlike classically developed NWV tools. This flexibility enables quantum computers to benefit irregular or atypical networks, where currently existing NWV may struggle to apply. Furthermore, while the discussed methods establish an upper limit on quantum algorithm runtime, combining algorithms like Simon’s with Grover’s—creating an \em{amplified Grover}—can expedite the discovery of biased solutions \cite{BrassardHoyer} potentially giving additional insight to property being investigated. Given the developing state of the field, the absence of a lower bound suggests potential for numerous optimizations to further expedite NWV processes.
    \begin{myitemize}
        \item NetDice: multiflow
        \item Packet-Header Analysis: timing / hop constraints
    
    \end{myitemize}
    \item Classical Success where quantum fails
    \begin{myitemize}
        \item Packet Header Analysis: Infinite loops
    \end{myitemize}

    \item Where both fail
    \begin{myitemize}
        \item Large input space needed: 
        \begin{myitemize}
            \item Classical needs sufficient structure: not clear always exists: SMT "works" but complaints is that it's too slow       
            \item Quantum might succeed but need to find structure, unstructured search not powerful enough
        \end{myitemize}
    \end{myitemize}
\end{myitemize}


